Classification of cohomogeneity-one actions on symmetric spaces of noncompact type

We complete the classification of isometric cohomogeneity-one actions on all symmetric spaces of noncompact type up to orbit equivalence.

==> other_stuff/intro__nonalphabetical_order_.tex <==
A proper isometric action of a Lie group $G$ on a connected Riemannian manifold $M$ is said to be of \textit{cohomogeneity one} if it has an orbit of codimension one. Cohomogeneity-one actions have been in the limelight because they can be used to construct Riemannian metrics with special properties: for instance, Einstein metrics, metrics with special holonomy, or metrics of positive sectional curvature (\cite{berard-bergery_cohomogeneity_one,böhm_C1_einstein,bryant_salamon_c1_g2_spin7,grove_wilking_ziller_pos_curv_c1}). One usually starts with a cohomogeneity-one action $G \curvearrowright M$ and dilates the existing metric $g$ along the orbits of $G$ to produce a new $G$-invariant metric, which might retain some properties of $g$ or gain new ones. Since most geometric structures on manifolds are governed by systems of partial differential equations, one can take advantage of the following principle: if a system of PDEs is invariant under a cohomogeneity-one action, it can be reduced to ODEs. For example, this can be applied to the Ricci flow, since it preserves isometries and hence the property of a metric of being invariant under a cohomogeneity-one action (see, e.g., \cite{bettiol_krishnan_4dim_C1_nonnegative,bettiol_krishnan_4dim_C1_positive}). Cohomogeneity-one actions are also an important object of study in submanifold geometry, since their principal orbits are homogeneous hypersurfaces and thus are isoparametric and have constant principal curvatures. Besides, cohomogeneity-one actions are one of the chief examples of hyperpolar (and hence polar) actions. Originally, these attracted interest due to their applications to topology: in \cite{bott_variationally_complete,bott_samelson_variationally_complete}, Bott and Samelson studied so-called variationally complete actions on symmetric spaces, which enabled them to apply Morse theory to the spaces of loops and paths on the ambient space; and in \cite{conlon_hyperpolar_implies_variationally_complete}, Conlon showed that hyperpolar actions are variationally complete.

Due to their prominence, it is natural to ask, what are all possible cohomogeneity-one actions on a given Riemannian manifold? This becomes a classification problem when we set a suitable geometric notion of equivalence: two actions are called \textit{orbit-equivalent} if there is an ambient isometry identifying their orbits. This problem is essentially equivalent to classifying homogeneous hypersurfaces up to isometric congruence. In this paper, by \textit{classification} we mean providing a complete and explicit list of actions up to orbit-equivalence---but we do allow some actions in the resulting list to be orbit-equivalent to each other. Figuring out exactly which ones are is referred to as the \textit{problem of congruence}; we do not pursue it here, although we will make occasional remarks about it along the way. 

The existence of at least one cohomogeneity-one action (from now on, \textit{C1-action}) implies a large isometry group, so it is sensible to first pose the classification problem for homogeneous spaces and in particular their most well-studied subclass of symmetric spaces. Historically, the first two symmetric spaces where the problem was solved were the Euclidean space $\E^n$ and the real hyperbolic space $\R H^n$. In them, it follows from the classification of isoparametric hypersurfaces---which all turn out to be homogeneous---by Somigliana, Levi-Civita, and Segre for $\E^n$ (\cite{somigliana_isoparametric,levi-civita_isoparametric,segre_isoparametric}) and by Cartan for $\R H^n$ (\cite{cartan_isoparametric}). The same approach does not work as smoothly for the sphere: famously, there are plenty of inhomogeneous isoparametric hypersurfaces in $\S^n$, but more importantly, the classification of isoparametric hypersurfaces in spheres still appears to be unfinished (see \cite{siffert_isoparam}). In \cite{hsiang_lawson}, Hsiang and Lawson proved that every C1-action on $\S^n$ is orbit-equivalent to the action induced by the isotropy representation of a symmetric space of rank 2 and dimension $n+1$. C1-actions on the other simply connected compact symmetric spaces---that is, on the projective spaces over the real division algebras $\C, \H$, and $\Oo$---were classified by Takagi (\cite{takagi_C1}), D'Atri (\cite{d'atri_C1_HP^n}), and Iwata (\cite{iwata_C1_HP^n,iwata_C1_OP^2}). In \cite{kollross_hyperpolar_c1_classification}, Kollross classified C1-actions on all irreducible symmetric spaces of compact type. His proof relied on Dynkin's classification of maximal subgroups of semisimple Lie groups (\cite{dynkin_subgroups_classical_english,dynkin_subalgebras_english}). In particular, Kollross showed that the moduli space of C1-actions on any such space is finite. On reducible symmetric spaces of compact type, the classification problem is still open.

On the other hand, the story of C1-actions on symmetric spaces of \textit{noncompact} type has been much more intricate and convoluted. The reason for this is that, informally speaking, noncompact semisimple Lie groups have ``way more" subgroups than compact ones. Excluding Cartan's classification for $\R H^n$, the story essentially begins with \cite{berndt_bruck}, where Berndt and Br\"{u}ck constructed a plethora of new examples of C1-actions on symmetric spaces of noncompact type and rank one. In particular, they obtained a one-parameter family of mutually orbit-non-equivalent C1-actions on the complex hyperbolic space $\C H^n$, thus showing that the moduli space of such actions can be not only infinite but even nondiscrete. Berndt and Br\"{u}ck's main tool was a novel method that allows one to construct C1-actions on a given space by solving a certain problem in the representation theory of reductive groups. They went on to solve that problem for $\C H^n$ and the Cayley hyperbolic plane $\Oo H^2$ but left the case of the quaternionic hyperbolic space $\H H^n$ open as it led to a pretty elaborate problem in quaternion algebra.

A C1-action on a symmetric space of noncompact type can have either one or zero singular orbits. In \cite{berndt_tamaru_foliations}, Berndt and Tamaru classified C1-actions without singular orbits on all irreducible symmetric spaces of noncompact type. They discovered that there are two distinct types of such actions: a continuous family parametrized by the projectivization of a maximal flat in $M$, and a discrete family parametrized by the simple roots of the restricted root system of $M$. They also solved the problem of congruence for these actions. In a later article \cite{hyperpolar_homogeneous_foliations} with D\'{i}az-Ramos, they generalized that result and classified homogeneous hyperpolar foliations on all symmetric spaces of noncompact type. In particular, that extends the classification in \cite{berndt_tamaru_foliations} to reducible spaces. In \cite{solonenko_foliations}, the first author also solved the problem of congruence in the reducible case. Berndt and Tamaru made another advancement in \cite{berndt_tamaru_totally_geodesic_singular_orbit}: they classified C1-actions with a totally geodesic singular orbit on all irreducible symmetric spaces of noncompact type. They showed that such an orbit is almost always a reflective submanifold and then used the classification of those obtained by Leung in \cite{leung_classification_of_reflective_submanifolds,leung_congruence}. Later in \cite{berndt_tamaru_rank_one}, Berndt and Tamaru proved that, in rank one, every C1-action with a non-totally-geodesic singular orbit arises via the construction method introduced by Berndt and Br\"{u}ck. As a consequence, that completed the classification for $\C H^n$ and $\Oo H^2$. The aforementioned quaternion algebra problem was solved much later in \cite{protohomogeneous}, which concluded the classification for $\H H^n$ and thus all rank-one spaces.

The next big development occurred in \cite{berndt_tamaru_cohomogeneity_one}. In that paper, Berndt and Tamaru generalized the method for constructing C1-actions from \cite{berndt_bruck} to spaces of arbitrary rank---the resulting procedure was given the name \textit{nilpotent construction}. The gist of this method is as follows: given a space $M$, one constructs a series of representations of certain reductive subgroups of the isometry group $I(M)$; in each of those representations, one has to look for subspaces satisfying certain properties---each such subspace gives rise to a C1-action on $M$. We will refer to the problem of finding all such subspaces as the \textit{nilpotent construction problem}. Berndt and Tamaru also invented another procedure---called the \textit{canonical extension}---allowing one to construct actions on spaces of higher rank from those on their certain totally geodesic submanifolds called boundary components. Since a boundary component is itself a symmetric space of noncompact type, one gets an inductive procedure for extending C1-actions into higher rank. The main result of \cite{berndt_tamaru_cohomogeneity_one} asserts that, on any (possibly reducible) symmetric space of noncompact type, if a C1-action has a non-totally-geodesic singular orbit, it must arise via either the canonical extension or the nilpotent construction. One of the big underpinnings of that result was Mostow's description of maximal subalgebras of real semisimple Lie algebras in \cite{mostow_maximal_subgroups}. By that point, there remained only two obstacles on the path to full classification. The first of them was understanding C1-actions with a totally geodesic singular orbit on \textit{reducible} spaces. This problem was bypassed in \cite{DR_DV_Otero_C1} by means of Dynkin's structural result \cite[Th.\hspace{2pt}15.1]{dynkin_subalgebras_english} (see also \cite[Th.\hspace{2pt}2.1]{kollross_hyperpolar_c1_classification}) on maximal subalgebras of semisimple Lie algebras---which largely complements the one by Mostow.

To complete the classification, one is left to solve the nilpotent construction problem. To this day, this has only been done in rank one, on some spaces of rank two (\cite{berndt_tamaru_cohomogeneity_one,berndt_DV_C1_rank_2,solonenko_hypersurfaces}), as well as on $\SL(n,\R)/\SO(n), \, n \ge 3$ (\cite{DR_DV_Otero_C1}). The aim of the current article is to resolve this problem for all symmetric spaces of noncompact type and thus conclude the classification---see the \hyperlink{thm:main}{Main theorem} below.

We now briefly introduce the necessary context and lay out our main result. (For more details, see Sections \ref{sec:preliminaries} and \ref{sec:c1-actions}.) Let $M = G/K$ be a symmetric space of noncompact type, where $G = I^0(M)$ is the identity component of the isometry group of $M$ and $K$ is the isotropy group of some point $o \in M$. The isometry Lie algebra $\mk{g}$ splits into a Cartan decomposition $\mk{g} = \mk{k} \oplus \mk{p}$, where $\mk{k} = \Lie(K)$. If we write $\uptheta$ for the corresponding Cartan involution and $B$ for the Killing form of $\mk{g}$, then we can define an inner product on $\mk{g}$ by the formula $B_\uptheta(X,Y) = -B(X,\uptheta Y)$. Pick a maximal abelian subspace $\mk{a}$ in $\mk{p}$. This induces the restricted root space decomposition $\mk{g} = \mk{g}_0 \oplus \bigoplus_{\upalpha \in \Upsigma} \mk{g}_\upalpha$ with respect to the restricted root system $\Upsigma \subset \mk{a}^*$. We have $\mk{g}_0 = \mk{k}_0 \oplus \mk{a}$, where $\mk{k}_0$ is the centralizer of $\mk{a}$ in $\mk{k}$. Fix a choice of simple roots $\Uplambda \subset \Upsigma$; this yields a nilpotent subalgebra $\mk{n} = \bigoplus_{\upalpha \in \Upsigma^+} \mk{g}_\upalpha$ of $\mk{g}$ and an Iwasawa decomposition $\mk{g} = \mk{k} \oplus \mk{a} \oplus \mk{n}$.

Take a one-dimensional subspace $\ell \subseteq \mk{a}$ and consider $\mk{h}_\ell = (\mk{a} \ominus \ell) \oplus \mk{n}$, where the first summand stands for the orthogonal complement of $\ell$ in $\mk{a}$. This is a Lie subalgebra of $\mk{g}$, and its corresponding Lie subgroup $H_\ell$ acts on $M$ with cohomogeneity one and no singular orbits---hence its orbits induce a Riemannian foliation. Similarly, take a simple root $\upalpha_i \in \Uplambda$ and any one-dimensional subspace $\ell_{\upalpha_i} \subseteq \mk{g}_{\upalpha_i}$. Then $\mk{h}_{\upalpha_i} = \mk{a} \oplus (\mk{n} \ominus \ell_{\upalpha_i})$ is a Lie subalgebra of $\mk{g}$ whose corresponding Lie subgroup $H_{\upalpha_i}$ also acts on $M$ with cohomogeneity one and no singular orbits. A different choice of $\ell_{\upalpha_i}$ in $\mk{g}_{\upalpha_i}$ leads to an orbit-equivalent action.

Suppose for a moment that  $M = M_1 \times M_2$, where $M_1$ and $M_2$ are homothetic symmetric spaces of noncompact type and rank one, and write $\mk{g}_i$ for their isometry Lie algebras. Pick an isomorphism $\upvarphi \colon \mk{g}_1 \isoto \mk{g}_2$ and consider the diagonal subalgebra $\mk{g}_\upvarphi = \set{X + \upvarphi(X) \mid X \in \mk{g}_1} \subset \mk{g}_1 \oplus \mk{g}_2 = \mk{g}$. Then the corresponding connected Lie subgroup $G_\upvarphi \subset G_1 \times G_2 = G$ (here $G_i = I^0(M_i)$) acts on $M$ with cohomogeneity one and a totally geodesic singular orbit---we call this a \textit{diagonal C1-action} on $M$.

Coming back to a general $M$, take any subset $\Upphi \subseteq \Uplambda$ of simple roots. We can define a subspace $\mk{a}_\Upphi = \bigcap_{\upalpha \in \Upphi} \Ker(\upalpha)$ of $\mk{a}$ together with its centralizer $\mk{l}_\Upphi = Z_\mk{g}(\mk{a}_\Upphi)$ and the subalgebra $\mk{m}_\Upphi = \mk{l}_\Upphi \ominus \mk{a}_\Upphi$. The $o$-orbit of the connected Lie subgroup corresponding to $\mk{m}_\Upphi$ is called a \textit{boundary component} of $M$ and denoted by $B_\Upphi$. This is a totally geodesic submanifold and a symmetric space of noncompact type in its own right. Its restricted root system $\Upsigma_\Upphi$ can be realized as the root subsystem of $\Upsigma$ generated by $\Upphi$. Note that $\Upsigma_\Upphi$ inherits a choice $\Upphi$ of simple roots. This allows us to define a subalgebra $\mk{n}_\Upphi = \bigoplus_{\uplambda \in \Upsigma^+ \mysetminus \Upsigma_\Upphi^+} \mk{g}_\uplambda$. The isometry Lie algebra $\mk{g}'_\Upphi$ of $B_\Upphi$ can be realized as the subalgebra of $\mk{g}$ generated by $\mk{g}_\upalpha$ as $\upalpha$ runs through $\Upsigma_\Upphi$. The connected Lie subgroup of $G$ corresponding to $\mk{g}'_\Upphi$ is denoted by $G'_\Upphi$ and is a finite covering of $I^0(B_\Upphi)$. Let $H_\Upphi \subseteq G'_\Upphi$ be a Lie subgroup with Lie algebra $\mk{h}_\Upphi \subseteq \mk{g}'_\Upphi$. We can then define a subalgebra $\mk{h}_\Upphi^\Uplambda = \mk{h}_\Upphi \oplus \mk{a}_\Upphi \oplus \mk{n}_\Upphi$ of $\mk{g}$, whose corresponding connected Lie subgroup $H_\Upphi^\Uplambda \subseteq G$ acts on $M$ with the same cohomogeneity as that of $H_\Upphi \curvearrowright B_\Upphi$. This procedure is called the \textit{canonical extension}.

Write $\Uplambda = \set{\upalpha_1, \ldots, \upalpha_r}$, let $H^1, \ldots, H^r$ be the dual basis for $\mk{a}$, and denote $H^\Upphi = \sum_{\upalpha_i \in \Upphi} H^i$. The subalgebra $\mk{n}_\Upphi$ is graded: $\mk{n}_\Upphi = \bigoplus_{\upnu \ge 1} \mk{n}_\Upphi^\upnu$, where $\mk{n}_\Upphi^\upnu$ is the eigenspace of $\ad(H^\Upphi)$ in $\mk{n}_\Upphi$ with eigenvalue $\upnu$. Define $L_\Upphi = Z_G(\mk{a}_\Upphi)$ and $K_\Upphi = K \cap L_\Upphi$. The orbit $L_\Upphi \cdot o$ contains $B_\Upphi$ and is denoted by $F_\Upphi$. The adjoint representation of $K_\Upphi$ on $\mk{g}$ is orthogonal and preserves the grading on $\mk{n}_\Upphi$. For every subspace $\mk{w} \subseteq \mk{n}_\Upphi^1$, the sum $\mk{n}_{\Upphi,\mk{w}} = \mk{w} \oplus \bigoplus_{\upnu \ge 2} \mk{n}_\Upphi^\upnu$ is a subalgebra, and its corresponding Lie subgroup is denoted by $N_{\Upphi,\mk{w}}$. Such a subspace $\mk{w}$ is called \textit{admissible} if $N_{L_\Upphi}(\mk{w})$ acts transitively on $F_\Upphi$ and \textit{protohomogeneous} if $N_{K_\Upphi}(\mk{w})$ acts transitively on the unit sphere in $\mk{v} = \mk{n}_\Upphi^1 \ominus \mk{w}$ (see Remark \ref{rem:w_vs_v}). If $\mk{w}$ satisfies these conditions and has $\codim_{\mk{n}_\Upphi^1}(\mk{w}) \ge 2$, then the subgroup $N^0_{L_\Upphi}(\mk{w})N_{\Upphi,\mk{w}}$ acts on $M$ with cohomogeneity one and has a singular orbit of codimension equal to $\codim_{\mk{n}_\Upphi^1}(\mk{w})$. This is called the \textit{nilpotent construction}, and the problem of finding all such subspaces $\mk{w}$ is called the \textit{nilpotent construction problem}. Note that if two admissible and protohomogeneous subspaces $\mk{w}, \mk{w}' \subseteq \mk{n}_\Upphi^1$ differ by an element of $K_\Upphi$, they give rise to orbit-equivalent actions. For reasons to be explained in Section \ref{sec:c1-actions} (see Theorem \ref{thm:classification_of_c1_actions}), one only has to consider this problem when $\Upphi$ is of the form $\Uplambda \mysetminus \set{\upalpha_j}$ for some simple root $\upalpha_j$. In that case, it is customary to replace $\Upphi$ with $j$ in subscripts and superscripts---e.g., $\mk{a}_j$ instead of $\mk{a}_\Upphi$, $\mk{n}_{j,\mk{w}}$ instead of $\mk{n}_{\Upphi,\mk{w}}$, and so on. The nilpotent construction problem has only been solved for a handful of spaces, and only on five of them it has given rise to new C1-actions not obtainable via other methods described above. Let us go through each of them briefly.

For rank-one spaces, we have $\Uplambda = \set{\upalpha_1}$ and $\mk{n}_1^1 = \mk{g}_{\upalpha_1}$, and every subspace of $\mk{n}_1^1$ is trivially admissible. In this case, it is more convenient to describe $\mk{w}$ in terms of its orthogonal complement $\mk{v}$. If $M = \C H^{n+1}$, we have $\mk{n}_1^1 \simeq \C^n, \, K_1 \simeq \U(n)$, and the representation of $K_1$ on $\mk{n}_1^1$ is the tautological representation of the unitary group. It was shown in \cite{berndt_bruck} that $\mk{w} \subseteq \mk{n}_1^1$ is protohomogeneous if and only if for every nonzero $v \in \mk{v}$, the angle between $Jv$ (here $J$ is the complex structure on $\mk{n}_1^1 \simeq \C^n$) and $\mk{v}$ is a constant not depending on $v$; this angle is then called the \textit{K\"{a}hler angle} of $\mk{v}$. Such a subspace $\mk{v}$---and thus the resulting C1-action---is determined by its K\"{a}hler angle and dimension up to congruence by $\U(n)$. Disregarding those subspaces that lead to C1-actions with a totally geodesic singular orbit, we obtain from \cite{berndt_bruck} that the moduli space of C1-actions on $\C H^{n+1}$ coming from the nilpotent construction and no other method is given by $\bm{\mc{M}_{\C H^{n+1}}} = (0,\frac{\uppi}{2}) \times \set{2, 4, \ldots, 2 \lfloor \frac{n}{2} \rfloor} \hspace{1pt} \sqcup \hspace{1pt} \set{\frac{\uppi}{2}} \times \set{2, 3, \ldots, n}$. If $M = \H H^{n+1}$, the representation $K_1 \curvearrowright \mk{n}_1^1$ is equivalent to the standard representation $\Sp(n)\Sp(1) \curvearrowright \H^n$. In that same paper, Berndt and Br\"{u}ck devised a generalization of the notion of K\"{a}hler angle to real subspaces of $\H^n$, which they called the \textit{quaternion-K\"{a}hler angle}. This time, this is a \textit{triple} of angles $(\upvarphi_1, \upvarphi_2, \upvarphi_3) \in [0,\frac{\uppi}{2}]^3$. As was shown in \cite{protohomogeneous}, for every protohomogeneous subspace $\mk{w}$ of $\H^n$, $\mk{v}$ has constant quaternion-K\"{a}hler angle and is \textit{almost} determined by it together with its dimension up to $\Sp(n)\Sp(1)$: for certain angles and dimensions, there might be two noncongruent subspaces. Therefore, the moduli space $\bm{\mc{M}_{\H H^{n+1}}}$ of C1-actions on $\H H^{n+1}$ arising from the nilpotent construction but no other method is a certain subset of the disjoint union of a collection of cubes $[0,\frac{\uppi}{2}]^3$. That subset (as well as the corresponding subspaces) was given an explicit description in \cite{protohomogeneous} (see Theorem A therein). If $M = \Oo H^2$, the representation $K_1 \curvearrowright \mk{n}_1^1$ is equivalent to the spin representation $\Spin(7) \curvearrowright \R^8$. The corresponding protohomogeneous subspaces were classified in \cite{berndt_bruck,berndt_tamaru_rank_one}, and the resulting moduli space can be described as $\bm{\mc{M}_{\Oo H^2}} = \set{2,3,6,7} \hspace{1pt} \sqcup \hspace{1pt} [0,1] \times \set{4}$. For each of these rank-one spaces, the C1-action corresponding to $\mk{w}$ is given on the level of Lie algebras by $ \mk{h}_{1,\mk{w}} = N_{\mk{k}_0}(\mk{w}) \oplus \mk{a} \oplus \mk{w} \oplus \mk{g}_{2\upalpha_1}$. Finally, consider the rank-two spaces $\mm{G}_2^2/\SO(4)$ and $\mm{G}_2(\C)/\mm{G}_2$. Let us write $\Uplambda = \set{\upalpha_1, \upalpha_2}$, where $\upalpha_2$ is the short simple root. As shown in \cite{berndt_tamaru_cohomogeneity_one}, for either space, the nilpotent construction yields only one new C1-action, which corresponds to the choice $j = 2$ and $\mk{w} = \set{0}$; the corresponding subgroup $H_{2,0}$ has Lie algebra $\mk{h}_{2,0} = \mk{l}_2 \oplus \mk{n}_2^2 \oplus \mk{n}_2^3$.

Coming back to the general case one more time, suppose $M = \prod_i M_i$ is the de Rham decomposition of $M$. The group $G$ decomposes as $G = \prod_i G_i$, where $G_i = I^0(M_i)$. An isometric C1-action $H \curvearrowright M$ is called \textit{decomposable} if it is orbit-equivalent to the action of a subgroup of $G$ of the form $H_i \times \prod_{l \ne i} G_l$ for some $i$, where $H_i \subset G_i$. In this case, $H_i$ acts on the de Rham factor $M_i$ also with cohomogeneity one. We are now in a position to formulate the main result of the article.

\begin{mainthm}\hypertarget{thm:main}{}
    Let $M = G/K$ be a symmetric space of noncompact type and $H$ a connected Lie group acting on $M$ properly and isometrically. Then $H$ acts with cohomogeneity one if and only if its action is orbit-equivalent to one of the following:
    
    \begin{enumerate}[\normalfont (a)]
        \item\customlabel{thm:main:a}{a} The action of $H_\ell$ for some one-dimensional linear subspace $\ell \subseteq \mk{a}$.
        \item\customlabel{thm:main:b}{b} The action of $H_{\upalpha_i}$ for some simple root $\upalpha_i \in \Uplambda$.
        \item\customlabel{thm:main:c}{c} The canonical extension of a C1-action with a totally geodesic singular orbit on an irreducible boundary component $B_\Upphi$ of $M$.
        \item\customlabel{thm:main:d}{d} The canonical extension of a diagonal C1-action on a reducible rank-2 boundary component $B_\Upphi$ of $M$ whose de Rham factors are homothetic.
        \item\customlabel{thm:main:e}{e} A decomposable action $H_i \times \prod_{l \ne i} G_l \curvearrowright M_i \times \prod_{l \ne i} M_l = M$, where the de Rham factor $M_i$ and the action $H_i \curvearrowright M_i$ are one of the following:

        \begin{enumerate}[\normalfont (1)]
            \item\customlabel{thm:main:e:1}{1} $M_i$ is isometric to
            
            \begin{itemize}
                \item $\Gr^*(k,\C^{2k+n}) \; (k \ge 1, n \ge 2)$,
                \item $\SO(2n+1, \H)/\U(2n+1) \; (n \ge 2)$, or
                \item $\mm{E}_6^{-14}/\Spin(10)\U(1)$,
            \end{itemize}
            and $H_i \curvearrowright M_i$ is the canonical extension of an action on the boundary component $\C H^{n+1}$ {\normalfont(}resp., $\C H^3$ or $\C H^5${\normalfont)} of $M_i$ belonging to $\mc{M}_{\C H^{n+1}}$ {\normalfont(}resp., $\mc{M}_{\C H^3}$ or $\mc{M}_{\C H^5}${\normalfont)}.
            \item\customlabel{thm:main:e:2}{2} $M_i \simeq \Gr^*(k,\H^{2k+n}) \; (k,n \ge 1)$ and $H_i \curvearrowright M_i$ is the canonical extension of an action on the boundary component $\H H^{n+1}$ of $M_i$ belonging to $\mc{M}_{\H H^{n+1}}$.
            \item\customlabel{thm:main:e:3}{3} $M_i \simeq \Oo H^2$ and $H_i \curvearrowright M_i$ is an action belonging to $\mc{M}_{\Oo H^2}$.
            \item\customlabel{thm:main:e:4}{4} $M_i \simeq \mm{G}_2^2/\SO(4)$ and $H_i = H_{2,0}$.
            \item\customlabel{thm:main:e:5}{5} $M_i \simeq \mm{G}_2(\C)/\mm{G}_2$ and $H_i = H_{2,0}$.
        \end{enumerate}
    \end{enumerate}
\end{mainthm}

Notice that the actions in \eqref{thm:main:b} and \eqref{thm:main:c} are also decomposable (see \cite[Th.\hspace{2pt}C]{DR_DV_Otero_C1}). It is worth pointing out that this theorem does not give a complete description of the moduli space of C1-actions yet, as one still needs to solve the problem of congruence for the actions described in \eqref{thm:main:a}-\eqref{thm:main:e}. We will make some occasional remarks about that in Section \ref{sec:c1-actions} (see also \cite[Rem.\hspace{2pt}1.1]{DR_DV_Otero_C1}), but we will not attempt to resolve the problem of congruence in general, since that would go beyond the scope of the paper.

Let us briefly lay out our strategy. In order to prove the \hyperlink{thm:main}{Main theorem}, we will have to resolve the nilpotent construction problem. As our first step, we will tackle the admissibility condition on the subspace $\mk{w}$---which has to do with \textit{transitive} actions on symmetric spaces. In the compact irreducible case, such actions were explicitly classified by Onishchik in \cite{onishchik_transitive}. There is little hope of getting a similar result in the noncompact case, as the list would be infinite for most spaces. As a substitute, we obtain a general structural result asserting that any Lie group acting transitively and isometrically on a symmetric space of noncompact type contains a skeleton of a very specific form.

\begin{thmA}\label{thm:B}\hspace{-5pt}\footnote{In the special cases of $\R H^n$ and $\C H^n$, a similar result was obtained in \cite[Th.\hspace{2pt}3.1, 4.1]{transitive_CH^n}}
    Let $M = G/K$ be a symmetric space of noncompact type and $H \subseteq G$ a Lie subgroup acting on $M$ transitively. Then there exist an Iwasawa decomposition $\mk{g} = \mk{k} \oplus \mk{a} \oplus \mk{n}$ and a maximal abelian subspace $\mk{t}_0 \subseteq \mk{k}_0$ such that the Lie algebra $\mk{h}$ of $H$ contains a solvable subalgebra of the form $V \oplus \mk{n}$, where $V \subseteq \mk{t}_0 \oplus \mk{a}$ projects surjectively onto $\mk{a}$.
\end{thmA}

Let us write $A$ and $N$ for the connected Lie subgroups of $G$ corresponding to $\mk{a}$ and $\mk{n}$, respectively. We have $G = KAN$, which is also called an Iwasawa decomposition. Informally speaking, Theorem \ref{thm:B} says that every transitive group of isometries of $M$ contains $N$ and ``almost contains" $A$ for some Iwasawa decomposition of $G$. In regard to the nilpotent construction, this theorem will let us show that the subspace $\mk{w}$ can always be assumed to respect the restricted root space decomposition of $\mk{g}$, which will significantly simplify the problem. Together with the protohomogeneity condition---or rather its Lie-algebraic reformulation---this will let us establish deep connections between the subspace $\mk{w}$ and root system $\Upsigma$ of $M$. For our next step, we observe that we should only care about actions that do not arise via any nontrivial canonical extension. We reinterpret this assumption in terms of how $\mk{w}$ interacts with the root spaces corresponding to the simple roots---which leads to very strong restrictions on $\Upsigma$, prohibits most choices of $\upalpha_j$, and rules out many spaces altogether solely based on their root systems. We then proceed to carry out a careful analysis of the singular orbit of $H_{j,\mk{w}}$ and its extrinsic geometry within the framework of the solvable model of $M$ (once again, see Section \ref{sec:preliminaries} for definitions and details). This will give us a much better understanding of whether the singular orbit is totally geodesic---and if it is, such an action can also be disregarded. Having done that, we will be able to rule out most of the remaining spaces simply by looking at their root multiplicities. At that stage, we will only be left to deal with spaces whose root systems are of type $\mm{B}_r$ or $\mm{BC}_r$. For these, we will have to resort to a more brute-force approach. We will examine the shape operators of the singular orbit using the Lie bracket relations between the root spaces of $\mk{g}$---and deduce that this orbit is bound to be totally geodesic, provided $r > 1$. Eventually, all these considerations will let us conclude that the nilpotent construction produces no actions other than the known examples or their canonical extensions, which will prove the \hyperlink{thm:main}{Main theorem}.

In our investigation of the nilpotent construction problem, we obtain two incidental results of independent interest. One of them is Theorem \ref{thm:B}, which we have already introduced above. The other side result concerns certain common classes of submanifolds of $M$ and gives them a useful uniform description---also in terms of an Iwasawa decomposition.

\begin{thmA}\label{thm:C}
    Let $M = G/K$ be a symmetric space of noncompact type and $S \subseteq M$ either of the following:
    \begin{enumerate}[\normalfont (a)]
        \item\customlabel{thm:C:a}{a} a complete connected totally geodesic submanifold,
        \item\customlabel{thm:C:b}{b} a singular orbit of a proper isometric C1-action.
    \end{enumerate}
    Then there exist an Iwasawa decomposition $G = KAN$ and a connected Lie subgroup $H \subseteq AN$ of the form $H = (H \cap A) \ltimes (H \cap N)$ such that $S = H \cdot o$.
\end{thmA}

Since $AN$ acts on $M$ simply transitively, we can think of $M$ as a solvable Lie group with a left-invariant metric. From this viewpoint, Theorem \ref{thm:C} asserts that every submanifold of $M$ of type \eqref{thm:C:a} or \eqref{thm:C:b} can be realized as a Lie subgroup---and is thus a solvmanifold. This makes studying extrinsic and intrinsic geometry of the submanifold considerably easier (see Subsection \ref{sec:preliminaries:extrinsic_geometry_cpc}). We expect that part \eqref{thm:C:a} of the theorem might aid the ongoing efforts to classify totally geodesic submanifolds in symmetric spaces (see \cite{t.g._exceptional_ss} and further references therein). Note that submanifolds in \eqref{thm:C:a} and \eqref{thm:C:b} are examples of homogeneous minimal submanifolds (for \eqref{thm:C:b}, this is shown in \cite[Prop.\hspace{2pt}3]{berndt_bruck}).

The article is organized as follows. Section \ref{sec:preliminaries} consists of preliminaries necessary for understanding everything that follows. In Section \ref{sec:c1-actions}, we talk in depth about the known types and methods of construction of C1-actions on symmetric spaces of noncompact type and discuss the current state of their classification. In Section \ref{sec:admissibility}, we deal with the admissibility condition in the nilpotent construction and prove Theorem \ref{thm:B}. This is the backbone of the whole paper that essentially renders the nilpotent construction solvable. Section \ref{sec:t.g._and_singular_orbit} is dedicated to the proof of Theorem~\ref{thm:C}. Finally, in Section \ref{sec:solving_the_NC}, we resolve the nilpotent construction problem and prove the \hyperlink{thm:main}{Main theorem}. 
%The whole section is essentially a careful analysis of the protohomogeneity condition and its interaction with the restricted root space decomposition---all in light of the results of Section \ref{sec:admissibility}.

\textbf{Acknowledgments.} The authors are indebted to Miguel Dom\'{i}nguez-V\'{a}zquez for his countless comments and suggestions, as well as to Tom\'{a}s Otero for his fruitful feedback on Section \ref{sec:admissibility}. The first author is particularly grateful to Miguel for organizing his visit to Santiago de Compostela in May 2024, which largely kick-started the project that led to this paper. I am also thankful to J\"{u}rgen Berndt for introducing me to the study of C1-actions and guiding me through it over the years of my PhD. Finally, we would like to thank Hiroshi Tamaru, Alberto Rodr\'{i}guez-V\'{a}zquez, and Jos\'{e} Carlos D\'{i}az-Ramos for sharing their insights and valuable advice.

==> other_stuff/preliminaries__nonalphabetical_order_.tex <==
This section serves as a collection of preliminaries required to understand the rest of the article. We begin with a brief refresher on some aspects of the theory of symmetric spaces of noncompact type in Subsection \ref{sec:preliminaries:symmetric_spaces_of_nc}. After that, in Subsection \ref{sec:preliminaries:parabolic}, we give a quick overview of the theory of parabolic subgroups of real semisimple Lie groups. Lastly, in Subsection \ref{sec:preliminaries:extrinsic_geometry_cpc}, we talk about a certain type of homogeneous submanifolds in symmetric spaces of noncompact type, whose extrinsic geometry such as shape operators can be studied effectively by means of the Iwasawa and restricted root space decompositions.

\subsection{Symmetric spaces of noncompact type}\label{sec:preliminaries:symmetric_spaces_of_nc}

Let $M$ be a symmetric space of noncompact type represented by a Riemannian symmetric pair $(G,K)$ with $G$ a connected noncompact semisimple Lie group and $K \subset G$ a maximal compact subgroup. We will usually write this simply as ``let $M = G/K$ be a symmetric space of noncompact type".

\begin{rem}
    By representing $M$ as $G/K$, we have a distinguished base point $eK \in M$, whose isotropy group is $K$. However, in certain circumstances, it might be beneficial to change the base point to a new one, say $o \in M$, that is better positioned. In that case, if there is no confusion, we will sometimes commit a slight abuse of notation and reuse the letter $K$ for the isotropy group of the new point $o$. This is equivalent to replacing $K$ with a conjugate subgroup but keeping the letter.
\end{rem}

The \textit{ineffectiveness kernel} of $(G,K)$ is the subgroup $I$ of elements of $G$ that act on $M$ trivially. Note that this is a closed normal subgroup. When unambiguous, we will refer to its Lie algebra $\mk{i}$, which is an ideal of $\mk{g} = \Lie(G)$, as the \textit{ineffectiveness kernel} as well.

\begin{agr}
    From now on, whenever we have a symmetric space $M$ of noncompact type and write it as $M = G/K$, we assume by default that $(G,K)$ is an \textit{almost effective} Riemannian symmetric pair. This means that the ineffectiveness kernel $I \subset G$ is finite. It follows a posteriori that $K$ is compact and $I$ coincides with the center of $G$. We refer to \cite[Sect.\hspace{2pt}2.4.1]{solonenko_thesis} for details.
\end{agr}

Fix a base point $o \in M$. The subgroup $K = G_o$ is the fixed-point set of a unique involutive automorphism $\Uptheta$ of $G$. The corresponding automorphism $\uptheta$ of $\mk{g}$ is a Cartan involution, and we will denote its corresponding Cartan decomposition by $\mk{g} = \mk{k} \oplus \mk{p}$. Here $\mk{k} = \Ker(\Id_\mk{g}\hspace{-1pt} -\hspace{1.5pt} \uptheta) = \Lie(K)$ and $\mk{p} = \Ker(\Id_\mk{g}\hspace{-1pt} +\hspace{1.5pt} \uptheta)$. The reductive complement $\mk{p}$ gets naturally identified with $T_oM$ by sending $X \in \mk{p}$ to the value of its corresponding Killing vector field $\wh{X}$ at $o$. Having fixed $\uptheta$, we have a $K$-invariant inner product on $\mk{g}$ given by $B_\uptheta(X,Y) = -B(X,\uptheta Y)$, where $B$ is the Killing form. Throughout the article, we will use $B_\uptheta$ as a default inner product on $\mk{g}$. We will also denote it by $\cross{-}{-}_{B_\uptheta}$ or even $\cross{-}{-}$ if there is no ground for confusion. Given two subspaces $U \subseteq V \subseteq \mk{g}$, $V \ominus U$ stands for the orthogonal complement of $U$ inside $V$. The summands $\mk{k}$ and $\mk{p}$ are orthogonal with respect to both $B_\uptheta$ and $B$; $B_\uptheta$ coincides with $B$ on $\mk{p} \times \mk{p}$ and equals $-B$ on $\mk{k} \times \mk{k}$. Being a $K$-invariant inner product on $\mk{p} \cong T_oM$, $\restr{B_\uptheta}{\mk{p} \times \mk{p}}$ can be extended to a $G$-invariant Riemannian metric $g_B$ on $M$. This is called the \textit{Killing metric}; it is symmetric, does not depend on the choice of a base point, and can be obtained by rescaling the original metric $g$ along each de Rham factor of $M$---in fact, any $G$-invariant metric on $M$ can be obtained in this way (and is thus also symmetric). The Killing metric enjoys the following property: if two de Rham factors of $M$ are homothetic, then they are isometric with respect to $g_B$. In general, a $G$-invariant metric on $M$ satisfying this property is said to be \textit{almost Killing}. Almost Killing metrics have the largest isometry group (all equal to $I(M,g_B)$), of which $I(M,g)$ is an open subgroup; in particular, we always have $I^0(M,g) = I^0(M,g_B)$. It can be shown that $I(M,g_B)$ is naturally isomorphic to $\Aut(\mk{g})$ (see \cite[Sect.\hspace{2pt}3]{solonenko_automorphisms} for details).

Pick a maximal abelian subspace $\mk{a}$ in $\mk{p}$. Given $\upalpha \in \mk{a}^*$, we let
$$
\mk{g}_\upalpha = \set{X \in \mk{g} \mid [H,X] = \upalpha(H)X \; \text{for every} \; H \in \mk{a}},
$$
and we also put $\Upsigma = \left\{\upalpha \in \mk{a}^* \mysetminus \{0\} \mid \mk{g}_\upalpha \ne \{0\}\right\}$. This set is called the restricted root system of $\mk{g}$ (or $M$) and its elements are called restricted roots. These induce a restricted root space decomposition $\mk{g} = \mk{g}_0 \oplus \bigoplus_{\upalpha \in \Upsigma} \mk{g}_\upalpha$. The summands of this decomposition are all pairwise orthogonal with respect to $B_\uptheta$, and we can also decompose $\mk{g}_0 = \mk{k}_0 \oplus \mk{a}$, where $\mk{k}_0 = Z_\mk{k}(\mk{a})$. The dimension of $\mk{g}_\upalpha$ is called the \textit{multiplicity} of the root $\upalpha$. It is customary to denote $\Upsigma_0 = \Upsigma \cup \set{0}$. For any $\upalpha, \upbeta \in \Upsigma_0, \, \upalpha \ne - \upbeta$, we have $[\mk{g}_\upalpha, \mk{g}_\upbeta] = \mk{g}_{\upalpha + \upbeta}$. This implies that the adjoint representation of $\mk{k}_0$ on $\mk{g}$ preserves each root space $\mk{g}_\upalpha$. We can restrict $B_\uptheta$ to an inner product on $\mk{a}$ and use it to identify $\mk{a}$ with $\mk{a}^*$ in a standard way, which in turn induces an inner product on $\mk{a}^*$. With respect to this inner product, $\Upsigma$ becomes a root system in $\mk{a}^*$. We can pull each root $\upalpha \in \Upsigma$ back under the isomorphism $\mk{a} \isoto \mk{a}^*$ and define a vector $H_\upalpha \in \mk{a}$; in other words, $H_\upalpha$ is determined by $\cross{H_\upalpha}{H} = \upalpha(H) \defqe \bilin{\upalpha}{H}$ for every $H \in \mk{a}$.

We make a choice of positive roots $\Upsigma^+ \subset \Upsigma$ and write $\Uplambda = \set{\upalpha_1, \ldots, \upalpha_r}$ for the corresponding set of simple roots. This allows us to define a nilpotent subalgebra $\mk{n} = \bigoplus_{\upalpha \in \Upsigma^+} \mk{g}_\upalpha$, which leads to a vector space decomposition $\mk{g} = \mk{k} \oplus \mk{a} \oplus \mk{n}$, also known as an Iwasawa decomposition. We will write $\Upsigma^-$ for the set $-\Upsigma^+$ of negative roots and $\DD$ for the Dynkin diagram of $\Upsigma$. Any root $\upalpha \in \Upsigma^+$ can be written as $\upalpha = \sum_{i=1}^r n_i \upalpha_i$ with $n_i \in \Z_{\ge 0}$, and the positive integer $\height(\upalpha)= \sum_{i=1}^r n_i$ is called the \textit{height} of $\upalpha$. Since $\upalpha_1, \ldots, \upalpha_r$ form a basis for $\mk{a}^*$, we can introduce the dual basis $H^1, \ldots, H^r$ for $\mk{a}$; these vectors are determined by $\cross{H^i}{H_{\upalpha_j}} = \bilin{H^i}{\upalpha_j} = \updelta_{ij}$. By definition, if $\upalpha = \sum_{i=1}^r n_i \upalpha_i$, then $\bilin{H^i}{\upalpha} = n_i$. Given a root $\upalpha \in \Upsigma$, we denote $\mk{k_\upalpha} = \mk{k} \cap (\mk{g}_\upalpha \oplus \mk{g}_{-\upalpha})$ and $\mk{p_\upalpha} = \mk{p} \cap (\mk{g}_\upalpha \oplus \mk{g}_{-\upalpha})$. This leads to decompositions $\mk{k} = \mk{k}_0 \oplus \bigoplus_{\upalpha \in \Upsigma^+} \mk{k}_\upalpha$ and $\mk{p} = \mk{a} \oplus \bigoplus_{\upalpha \in \Upsigma^+} \mk{p}_\upalpha$. Notice that we have $\mk{g}_\upalpha \oplus \mk{g}_{-\upalpha} = \mk{k}_\upalpha \oplus \mk{p}_\upalpha$ for every $\upalpha \in \Upsigma$.

%A (weight-preserving) automorphism of $\Upsigma$ is a linear automorphism $f \colon \mk{a}^* \isoto \mk{a}^*$ that preserves $\Upsigma$ and respects the root integers and multiplicities, i.e., $n_{f(\upalpha)f(\upbeta)} = n_{\upalpha\upbeta}, \, \mult(f(\upalpha)) = \mult(\upalpha)$; the group of automorphisms of $\Upsigma$ is denoted by $\Aut^\mm{w}(\Upsigma)$. The Weyl subgroup $W(\Upsigma)$ is a normal subgroup of $\Aut^\mm{w}(\Upsigma)$. Going further, we denote the Dynkin diagram of $\Upsigma$ by $\DD$. We think of it as a weighted diagram by assigning to each vertex the multiplicity of the corresponding simple root. An automorphism of $\DD$ is said to be weight-preserving if it preserves the weights of the vertices; the group of such automorphisms is denoted by $\Aut^\mm{w}(\DD)$. Every automorphism of $\DD$ extends naturally to a linear automorphism of $\mk{a}^*$, and in fact we have $\Aut^\mm{w}(\Upsigma) = W(\Upsigma) \rtimes \Aut^\mm{w}(\DD)$. The connected components of $\DD$ correspond naturally to the de Rham factors of $M$. Two such components $\DD_i$ and $\DD_j$ may happen to be isomorphic (as weighted diagrams), which translates to the corresponding factors $M_i$ and $M_j$ being homothetic. We consider the subgroup $\Aut^\mm{w}(\DD)_M$ of $\Aut^\mm{w}(\DD)$ consisting of automorphisms $\upvarphi$ satisfying the following property: for each connected component $\DD_i$ of $\DD$, if $\upvarphi(\DD_i) = \DD_j$, then the corresponding de Rham factors $M_i$ and $M_j$ of $M$ are isometric. Informally speaking, these are the diagram symmetries of $\DD$ that can be lifted to isometries of $M$. For more details on this, see \cite{solonenko_automorphisms}. Note that $\Aut^\mm{w}(\DD)_M = \Aut^\mm{w}(\DD)$ if and only if the metric $g$ in almost Killing. Since the group $\Aut^\mm{w}(\Upsigma)$ acts on $\mk{a}^*$, it also acts naturally on $\mk{a}$; the same is thus true for its subgroups $\Aut^\mm{w}(\DD)$ and $\Aut^\mm{w}(\DD)_M$.

We write $A$ and $N$ for the connected Lie subgroups of $G$ corresponding to $\mk{a}$ and $\mk{n}$, respectively. These subgroups are closed and simply connected. The multiplication in $G$ yields a diffeomorphism $K \times A \times N \isoto G$, which is also called an Iwasawa decomposition. The Lie group $A$ normalizes $N$, so the semidirect product $A \ltimes N$ is a solvable subgroup of $G$. (We will normally shorten $A \ltimes N$ to just $AN$.) The action $AN \curvearrowright M$ is simply transitive and the metric pulled back from $M$ to $AN$ along the diffeomorphism $AN \isoto M, \, an \mapsto an \cdot o,$ is left-invariant, hence $M$ can be thought of as a simply connected solvable Lie group with a left-invariant metric---we call this the \textit{solvable model} of $M$. The orbit $A \cdot o$ is a maximal flat in $M$ and it is isometric to the Euclidean space $\E^r$, where $r = \dim(\mk{a})$ is the rank of $M$.

\subsection{Parabolic subalgebras and subgroups}\label{sec:preliminaries:parabolic}

The theory of parabolic subgroups of real semisimple Lie groups plays a pivotal role in the geometry of symmetric spaces of noncompact type because it yields a number of important decomposition results for the space itself, as well as for its isometry group. Among other things, these decompositions can be used to construct various homogeneous objects---like submanifolds or foliations---on the ambient space. They also underpin the two methods of constructing C1-actions with a non-totally-geodesic singular orbit. Here we lay out a brief exposition of the theory and refer to \cite{berndt_tamaru_cohomogeneity_one,solonenko_hypersurfaces,solonenko_thesis} for more details. For a deeper introduction, see \cite[Ch.\hspace{0.2pt}VII, Sect.\hspace{2pt}7]{knapp} and \cite[Sect.\hspace{2pt}13.2]{submanifolds_&_holonomy}.

Let $M = G/K$ be a symmetric space of noncompact type with a fixed choice of $o \in M, \mk{a} \subset \mk{p},$ and $\Upsigma^+ \subset \Upsigma$ as above. Fix any subset~$\Upphi \subseteq \Uplambda$.

\begin{itemize}
    \item We write $\Upsigma_\Upphi$ for the root subsystem of $\Upsigma$ generated by $\Upphi$. It inherits a choice of positive roots $\Upsigma_\Upphi^+ = \Upsigma_\Upphi \cap \Upsigma^+$.
    \item Next, define $\mk{a}_\Upphi = \bigcap_{\upalpha_i \in \Upphi} \Ker(\upalpha_i) = \bigoplus_{\upalpha_j \in \Uplambda \mysetminus \Upphi} \R H^j$ and $\mk{a}^\Upphi = \mk{a} \ominus \mk{a}_\Upphi = \bigoplus_{\upalpha_i \in \Upphi} \R H_{\upalpha_i}$.
    \item The subset $\Updelta_\Upphi = \Upsigma^+ \mysetminus \Upsigma_\Upphi^+$ can be split into parts: $\Updelta_\Upphi = \bigsqcup_{\upnu \ge 1} \Updelta_\Upphi^\upnu$, where $\Updelta_\Upphi^\upnu$ consists of the roots $\uplambda \in \Updelta_\Upphi$ with $\bilin{H^\Upphi}{\uplambda} = \upnu$, and $H^\Upphi = \sum_{\upalpha_j \in \Uplambda \mysetminus \Upphi} H^j$.
    \item Let $\mk{n}_\Upphi = \bigoplus_{\uplambda \in \Updelta_\Upphi} \mk{g}_\uplambda$. This nilpotent subalgebra is graded: $\mk{n}_\Upphi = \bigoplus_{\upnu \ge 1} \mk{n}_\Upphi^\upnu$, where $\mk{n}_\Upphi^\upnu = \bigoplus_{\uplambda \in \Updelta_\Upphi^\upnu} \mk{g}_\uplambda$ is the eigenspace of $\ad(H^\Upphi)$ in $\mk{n}_\Upphi$ with eigenvalue $\upnu$.
    \item Consider $\mk{l}_\Upphi = \mk{g}_0 \oplus \bigoplus_{\upalpha \in \Upsigma_\Upphi} \mk{g}_\upalpha$. This reductive subalgebra of $\mk{g}$ centralizes $\mk{a}_\Upphi$, normalizes $\mk{n}_\Upphi$, and preserves the grading on $\mk{n}_\Upphi$. In fact, one has $\mk{l}_\Upphi = Z_\mk{g}(\mk{a}_\Upphi)$.
    \item $\mk{q}_\Upphi = \mk{l}_\Upphi \loplus \mk{n}_\Upphi$ is a parabolic subalgebra of $\mk{g}$, and this semidirect sum is called a Chevalley decomposition. Every parabolic subalgebra of $\mk{g}$ is inner-conjugate to $\mk{q}_\Upphi$ for some choice of $\Upphi$. One can show that $\mk{n}_\Upphi$ is the nilradical of $\mk{q}_\Upphi$.
    \item Going further, let $\mk{m}_\Upphi = \mk{l}_\Upphi \ominus \mk{a}_\Upphi = \mk{k}_0 \oplus \mk{a}^\Upphi \oplus \bigoplus_{\upalpha \in \Upsigma_\Upphi} \mk{g}_\upalpha \subseteq \mk{l}_\Upphi$. This is also a reductive subalgebra of $\mk{g}$, and we have a direct sum decomposition $\mk{l}_\Upphi = \mk{m}_\Upphi \oplus \mk{a}_\Upphi$. The induced splitting $\mk{q}_\Upphi = (\mk{m}_\Upphi \oplus \mk{a}_\Upphi) \loplus \mk{n}_\Upphi$ is called a Langlands decomposition. We will normally omit the parentheses and simply write $\mk{m}_\Upphi \oplus \mk{a}_\Upphi \loplus \mk{n}_\Upphi$.
    \item The $\mk{k}$- and $\mk{p}$-parts of $\mk{m}_\Upphi$ are $\mk{k}_\Upphi = \mk{k}_0 \oplus \bigoplus_{\upalpha \in \Upsigma_\Upphi^+} \mk{k}_\upalpha$ and $\mk{b}_\Upphi = \mk{a}^\Upphi \oplus \bigoplus_{\upalpha \in \Upsigma_\Upphi^+} \mk{p}_\upalpha$, respectively.
    \item Being reductive, $\mk{m}_\Upphi$ is the direct sum of its center $\mk{z}_\Upphi \subseteq \mk{k}_0$ and its semisimple part $\mk{g}_\Upphi = [\mk{m}_\Upphi, \mk{m}_\Upphi] = [\mk{l}_\Upphi,\mk{l}_\Upphi]$.
    \item $\mk{g}_\Upphi$ splits as the direct sum of its compact and noncompact semisimple parts. The latter can be described as $\mk{g}'_\Upphi = [\mk{b}_\Upphi, \mk{b}_\Upphi] \oplus \mk{b}_\Upphi$, or alternatively, as the subalgebra of $\mk{g}$ generated by $\mk{g}_\upalpha, \, \upalpha \in \Upsigma_\Upphi$. The compact semisimple part of $\mk{g}_\Upphi$ is given by $Z_{\mk{k}_0}(\mk{g}'_\Upphi) \ominus \mk{z}_\Upphi$. The sum of the center of $\mk{m}_\Upphi$ and its compact semisimple part can thus be described as $Z_{\mk{k}_0}(\mk{g}'_\Upphi) = Z_{\mk{k}_0}(\mk{b}_\Upphi)$.
    \item $\mk{g}'_\Upphi$ comes with an Iwasawa decomposition: $\mk{g}'_\Upphi = \mk{k}^\Upphi \oplus \mk{a}^\Upphi \oplus \mk{n}^\Upphi$, where $\mk{k}^\Upphi = \mk{g}'_\Upphi \cap \mk{k}_\Upphi = \mk{g}'_\Upphi \cap \mk{k}$ and $\mk{n}^\Upphi = \mk{g}'_\Upphi \cap \mk{n} = \bigoplus_{\upalpha \in \Upsigma_\Upphi^+} \mk{g}_\upalpha$.
    \item We denote the $\mk{k}_0$-part of $\mk{g}'_\Upphi$ by $\mk{k}^\Upphi_0$. Note that \label{k_0_decomposition}
    $$
    \mk{k}_0 = Z_{\mk{k}_0}(\mk{g}'_\Upphi) \oplus \mk{k}^\Upphi_0 = \mk{z}_\Upphi \oplus (Z_{\mk{k}_0}(\mk{g}'_\Upphi) \ominus \mk{z}_\Upphi) \oplus \mk{k}^\Upphi_0.
    $$
    This is a direct sum of Lie algebras, and the summands are pairwise orthogonal with respect to $B_\uptheta$ (or $B$).
    \item The connected (closed) Lie subgroups of $G$ corresponding to $\mk{g}'_\Upphi, \mk{a}_\Upphi,$ and $\mk{n}_\Upphi$ are denoted by $G'_\Upphi, A_\Upphi,$ and $N_\Upphi$, respectively. Furthermore, we define:
    $$
    \hspace{6.5ex} L_\Upphi = Z_G(\mk{a}_\Upphi), \quad Q_\Upphi = L_\Upphi \ltimes N_\Upphi = N_G(\mk{q}_\Upphi), \quad K_\Upphi = K \cap L_\Upphi, \quad M_\Upphi = K_\Upphi G'_\Upphi.
    $$
    These are closed subgroups of $G$ with Lie algebras $\mk{l}_\Upphi, \mk{q}_\Upphi, \mk{k}_\Upphi,$ and $\mk{m}_\Upphi$, respectively. We have a direct product decomposition $L_\Upphi = M_\Upphi \times A_\Upphi$. The decompositions $Q_\Upphi = L_\Upphi \ltimes N_\Upphi$ and $Q_\Upphi = (M_\Upphi \times A_\Upphi) \ltimes N_\Upphi \defqe M_\Upphi \times A_\Upphi \ltimes N_\Upphi$ are also called Chevalley and Langlands decompositions of the parabolic subgroup $Q_\Upphi$, respectively. The adjoint representation of $L_\Upphi$ on $\mk{n}_\Upphi$ respects its grading. If we write $K^\Upphi, A^\Upphi,$ and $N^\Upphi$ for the connected Lie subgroups of $G'_\Upphi$ with Lie algebras $\mk{k}^\Upphi, \mk{a}^\Upphi,$ and $\mk{n}^\Upphi$, respectively, then we have a global Iwasawa decomposition $G'_\Upphi = K^\Upphi A^\Upphi N^\Upphi$.
    \item The orbit $B_\Upphi = G'_\Upphi \ccdot o = M_\Upphi \ccdot o$ is a \textit{boundary component} of $M$; it is a totally geodesic submanifold (corresponding to the Lie triple system $\mk{b}_\Upphi$) and itself a symmetric space of noncompact type and rank $r_\Upphi = |\Upphi|$. We can think of its Dynkin diagram $\DD_\Upphi$ as the subdiagram of $\DD$ spanned by the nodes corresponding to the roots in $\Upphi$. This space is represented by the almost effective Riemannian symmetric pair $(G'_\Upphi, K^\Upphi)$, as well as by the Riemannian symmetric pair $(M^0_\Upphi, K^0_\Upphi)$. Note that the latter has ineffectiveness kernel $Z_{\mk{k}_0}(\mk{g}'_\Upphi)$, which is compact. 
    \item The Langlands decomposition of $Q_\Upphi$ induces---via the transitive action $Q_\Upphi \curvearrowright M$---a horospherical decomposition $B_\Upphi \times A_\Upphi \times N_\Upphi \cong M$ (just a diffeomorphism). We can summarize this with the following diagram:
    \begin{equation*}
    \begin{tikzcd}
    M_\Upphi \times A_\Upphi \ltimes N_\Upphi \ar[r, "\sim" yshift = -0.2ex] \ar[d, twoheadrightarrow] & Q_\Upphi \ar[d, twoheadrightarrow] \ar[dr, twoheadrightarrow] \\
    B_\Upphi \times A_\Upphi \times N_\Upphi \ar[r, "\sim" yshift = -0.2ex] & Q_\Upphi/K_\Upphi \ar[r, "\sim" yshift = -0.2ex] & M
    \end{tikzcd}
    \end{equation*}
    With respect to the Langlands and horospherical decompositions, the action of $Q_\Upphi$ on $M$ can be written as:
    \begin{gather}\label{horospherical_decomposition_action}
    M_\Upphi \times A_\Upphi \ltimes N_\Upphi \curvearrowright B_\Upphi \times A_\Upphi \times N_\Upphi, \nonumber \\
    (m,a,n) \cdot (m' \cdot o,a',n') = ((mm') \cdot o,aa',(m'a')^{-1} n (m'a') n').
    \end{gather}
    \item The submanifold $F_\Upphi = L_\Upphi \cdot o \cong B_\Upphi \times A_\Upphi \subseteq M$ is also totally geodesic and is a symmetric space of rank $r$ with an $(r-r_\Upphi)$-dimensional flat factor; its splitting into the product of $B_\Upphi$ and $A_\Upphi \cong A_\Upphi \cdot o$ is a Riemannian product decomposition. For lack of a better word, we call $F_\Upphi$ an \textit{extended boundary component}. It corresponds to the Lie triple system $\mk{f}_\Upphi = \mk{b}_\Upphi \oplus \mk{a}_\Upphi$.
\end{itemize}

We will be mostly interested in the situations where $\Upphi$ is of the form $\Uplambda \mysetminus \set{\upalpha_j}$ for some simple root $\upalpha_j$. In that case, in all of the objects defined above, we simply replace the subscript or superscript $\Upphi$ with $j$; we also write $\Uplambda_j = \Uplambda \mysetminus \set{\upalpha_j}$. We then have $H^\Upphi = H^j$, and for each $\upalpha \in \Upsigma^+$, $\bilin{\upalpha}{H^j}$ gives the coefficient corresponding to $\upalpha_j$ in the expression of $\upalpha$ with respect to the simple system $\Uplambda$. Hence, the set $\Updelta_j^1$ can be described as
\begin{equation}\label{equation:levelone:string}
\Updelta_j^1 = \Bigl\{ \upalpha_j + \sum_{i \ne j} n_i \upalpha_i \in \Upsigma^+ \mid n_i \in \Z_{\ge 0} \Bigr\}.   
\end{equation}
In Section \ref{sec:solving_the_NC} we will need to determine explicitly the set $\Updelta_j^1$ for some particular choices of $\upalpha_j$. In order to do so, we will make use of the following generalization of the classical notion of a root string. Let $\Upphi \subseteq \Uplambda$ once again be an arbitrary subset of simple roots, and let $\uplambda \in \Upsigma$ be any root. We define the \emph{$\Upphi$-string of $\uplambda$} as the set of all the elements of $\Upsigma_0$ of the form $\uplambda + \sum_{\upalpha_i \in \Upphi} n_i \upalpha_i$ with $n_i \in \mathbb{Z}$. This notion of string was introduced by the second author in~\cite{sanmartin-strings}, where he also calculated all possible $\Upphi$-strings for all choices of $\Upsigma, \Upphi,$ and $\uplambda$. The base idea of that computation is simple: if $\uplambda$ is the root of minimum height in its $\Upphi$-string, then $\Upphi \cup \{ \uplambda \}$ is a simple system for the root subsystem $\Upsigma_{\Upphi, \uplambda} = \vspan_\Z(\Upphi \cup \{ \uplambda \}) \cap \Upsigma$ of $\Upsigma$. Note that for such $\uplambda$, every root $\uplambda + \sum_{\upalpha_i \in \Upphi} n_i \upalpha_i$ in the $\Upphi$-string has all $n_i$ nonnegative (see \cite[Prop.\hspace{2pt}2.49]{knapp}). The argument is then based on calculating explicitly the $\Upphi$-string of $\uplambda$ for any possible pair~$(\Upsigma, \Upsigma_{\Upphi, \uplambda})$. Under this new perspective, $\Updelta_j^1$ is nothing but the $\Uplambda_j$-string of $\upalpha_j$, as one can see from~\eqref{equation:levelone:string} and the fact that $\upalpha_j$ has minimum height in its $\Uplambda_j$-string. Hence, for any root system $\Upsigma$ and any choice of $j$, we have an explicit description of $\Updelta_j^1$. We will make great use of that in Section \ref{sec:solving_the_NC}.

\subsection{The extrinsic geometry of singular orbits}\label{sec:preliminaries:extrinsic_geometry_cpc}

As we have explained, any symmetric space $M$ of noncompact type can be regarded as a solvable Lie group $AN$ endowed with a certain left-invariant metric. One of the key underpinnings of this work is the fact that the singular orbit of a nilpotent construction action\footnote{Recall from Theorem \ref{thm:C} that this is in fact true for any C1-action. We will show this in Section \ref{sec:t.g._and_singular_orbit}.} on $M$ can always be realized as a Lie subgroup of $AN$. This property singles out a very special class of submanifolds of $M$, whose geometry is tied particularly closely to the structure of the isometry Lie algebra $\mk{g}$. In the following lines, we introduce a few tools that will help us study the extrinsic geometry of such submanifolds.

Let $M = G/K$ be a symmetric space of noncompact type. In this subsection, we assume that the metric on $M$ is Killing (see Remark \ref{rem:choice_of_metric}). As usual, we fix a point $o \in M$, a maximal abelian subspace $\mk{a} \subset \mk{p}$, and a set of positive roots $\Upsigma^+ \subset \Upsigma$. These choices give rise to an Iwasawa decomposition $G = KAN$ and an identification $AN \cong M$. The isomorphism $\mk{a} \oplus \mk{n} \isoto T_oM \cong \mk{p}$ is given simply by the projection onto $\mk{p}$ along $\mk{k}$. As follows from the proof of~\cite[Prop.\hspace{2pt}4.4]{tamaru_parabolic_Einstein}, the induced left-invariant metric on $AN$ is related to the inner product on $\mk{g}$ via the equation
\begin{equation}\label{equation:inner:relation:b:theta:an}
\cross{X}{Y}_{AN} = \cross{X_\mk{a}}{Y_\mk{a}}_{B_\uptheta} +\frac{1}{2} \cross{X_\mk{n}}{Y_\mk{n}}_{B_\uptheta} \quad \text{for any $X$, $Y \in \mk{a} \oplus \mk{n}$},
\end{equation}
where $\mk{a}$ and $\mk{n}$ in the subscript denote the $\mk{a}$- and $\mk{n}$-components of a vector, respectively. Since $\mk{a}$ and $\mk{n}$ are mutually orthogonal with respect to both inner products, we see from \eqref{equation:inner:relation:b:theta:an} that $\cross{X}{Y}_{AN} = \cross{X}{Y}_{B_\uptheta}$ whenever $X$ or $Y$ lies in $\mk{a}$; similarly, $\cross{X}{Y}_{AN} = \frac{1}{2}\cross{X}{Y}_{B_\uptheta}$ if $X$ or $Y$ lies in $\mk{n}$. The Levi-Civita connection on $AN$ also admits a neat expression. First, we need the following simple equality:
\begin{equation}\label{equation:inner:b:theta}
\cross{\ad(X) Y}{Z}_{B_\uptheta} = - \cross{Y}{\ad(\uptheta X) Z}_{B_\uptheta} \quad \text{for any $X$, $Y$, $Z \in \mk{g}$}.
\end{equation}
Combining this with the Koszul formula and \eqref{equation:inner:relation:b:theta:an} leads to:
\begin{equation}\label{equation:levi:civita:connection:an}
\cross{\nabla_X Y}{Z}_{AN} = \frac{1}{4} \cross{[X,Y] + [\uptheta X, Y] - [X, \uptheta Y]}{Z}_{B_\uptheta} \quad \text{for any $X$, $Y$, $Z \in \mk{a} \oplus \mk{n}$}.
\end{equation}
Now, let $H$ be a connected Lie subgroup of $AN$ with Lie algebra $\mk{h}$. Under the identification between $M$ and $AN$, the orbit $H \cdot o$ corresponds to $H$, the tangent space $T_o(H \cdot o)$ becomes $\mk{h}$, and the normal space $N_o(H \cdot o)$ becomes $\mk{v} = (\mk{a} \oplus \mk{n}) \ominus \mk{h}$, where the orthogonal complement is taken with respect to $\cross{-}{-}_{AN}$. We would like to have a handy description of the shape operators of $H \cdot o$. Since this is a homogeneous submanifold, it suffices to examine its shape operators only at $o$.
\begin{lem}\label{lem:AN_shape_operators_general}
    Given $\upxi \in \mk{v}$, the shape operator $\mc{A}_\upxi$ of $H \cdot o$ at $o$ is given by the following formula:
    \begin{equation}\label{AN_shape_operators_general}
        \cross{\mc{A}_\upxi X}{Y}_{AN} = \frac{1}{4}\cross{[\upxi,X] - [\uptheta\upxi,X]}{Y}_{B_\uptheta} \quad \text{for any $X, Y \in \mk{h}$}.
    \end{equation} 
\end{lem}

\begin{proof}
    By definition, $\mc{A}_\upxi X = -(\nabla_X \upxi)^\top$, where $\top$ denotes the orthogonal projection to $\mk{h}$ along $\mk{v}$. Given $Y \in \mk{h}$, we use \eqref{equation:levi:civita:connection:an} to compute:
    $$
    \cross{\mc{A}_\upxi X}{Y}_{AN} = -\cross{(\nabla_X \upxi)^\top}{Y}_{AN} = -\cross{\nabla_X \upxi}{Y}_{AN} = \frac{1}{4} \cross{[\upxi,X] - [\uptheta X, \upxi] - [\uptheta \upxi,X]}{Y}_{B_\uptheta}.
    $$
    By comparing this to \eqref{AN_shape_operators_general}, it only remains to show that $\cross{[\uptheta X, \upxi]}{Y}_{B_\uptheta} = 0$. We calculate:
    $$
    \cross{[\uptheta X, \upxi]}{Y}_{B_\uptheta} = -\cross{\upxi}{[X,Y]}_{B_\uptheta} = -\cross{\upxi}{[X,Y]}_{AN} = 0.
    $$
    Here the first equality follows from \eqref{equation:inner:b:theta}, the second from the fact that $[X,Y] \in \mk{n}$, and the last one from $[X,Y] \in \mk{h}$. This completes the proof.
\end{proof}
Formula \eqref{AN_shape_operators_general} can be simplified still further provided we know some additional information about $\mk{h}$: for example, if $\mk{h} = (\mk{h} \cap \mk{a}) \loplus (\mk{h} \cap \mk{n})$ (which is often the case, see Theorem \ref{thm:C}) or if $\mk{h}$ contains nonzero vectors lying in a single root space. We will see a particular instance of that in the context of the nilpotent construction in Section \ref{sec:solving_the_NC} (see Proposition \ref{proposition:shape:orbit:an}). As a preparation for that, we need the following two results, which provide an insight into how different root spaces behave with respect to the Lie bracket.

\begin{lem}\label{lemma:a:k0} 
 Let $\upalpha \in \Sigma^{+}$, and let $X,Y \in \mk{g}_{\upalpha}$ be orthogonal. Then:
\begin{enumerate}[\normalfont (a)]
\item\customlabel{lemma:a:k0:1}{a} $[\uptheta X, X] = 2 ||X||^2_{AN} H_{\upalpha} = ||X||^2_{B_{\uptheta}} H_{\upalpha}$.
\item\customlabel{lemma:a:k0:2}{b} $[\uptheta X, Y] \in \mk{k}_0$.
\end{enumerate} 
\end{lem}

For a proof, see \cite[Lem.\hspace{2pt}2.3]{berndt_SL_CPC}. Note that we do not need to specify whether $X$ and $Y$ are orthogonal with respect to $\cross{-}{-}_{AN}$ or $B_\uptheta$, as those are proportional on $\mk{g}_\upalpha$.

\begin{lem}\label{lem:string_injective}
    Let $\upalpha,\upbeta \in \Upsigma$ be non-proportional roots and suppose that the $\upbeta$-string of $\upalpha$ has the form $\set{\upalpha, \upalpha + \upbeta, \ldots, \upalpha + m\upbeta}$ for some positive integer $m$. Then for any nonzero $X \in \mk{g}_\upbeta$ and any $1 \le k \le m$, the operator $\ad(X)^k \colon \mk{g}_\upalpha \to \mk{g}_{\upalpha + k\upbeta}$ is injective.
\end{lem}

\begin{proof}
    By choosing a different system of simple roots if necessary, we may assume without loss of generality that both $\upalpha$ and $\upbeta$ are positive. It follows from \cite[Prop.\hspace{2pt}2.48]{knapp} that $m \in \set{1,2,3}$. The case of $k=1$ (and any $m$) was done in \cite[Lem.\hspace{2pt}2.4(i)]{berndt_SL_CPC}, and the case $k = m = 2$ was shown in Proposition 4.2(iv) of the same paper. Therefore, we only need to deal with\footnote{This can only occur when the irreducible component of $\Upsigma$ containing $\upalpha$ and $\upbeta$ is isomorphic to $\mm{G}_2$.} $m = 3, \, k = 2,3$. Take a nonzero vector $Y \in \mk{g}_\upalpha$. By combining \cite[Lem.\hspace{2pt}2.4]{berndt_SL_CPC} with \cite[Prop.\hspace{2pt}2.48(g)]{knapp}, we obtain that $\ad(\uptheta X) \circ \ad(X)^3(Y)$ is a nonzero multiple of $\ad(X)^2(Y)$, and $\ad(\uptheta X) \circ \ad(X)^2(Y)$ is a nonzero multiple of $\ad(X)(Y)$. But we already know that this latter vector is nonzero. Consequently, $\ad(X)^2(Y)$ must be nonzero, and hence so does $\ad(X)^3(Y)$. This concludes the proof.
\end{proof}

In Section \ref{sec:solving_the_NC}, we will constantly use another important property of singular orbits of C1-actions: their principal curvatures, counted with multiplicities, do not depend on the normal unit direction. More rigorously, given such an orbit $S \subset M$ and two normal unit vectors $\upxi, \upnu \in NS$ (possibly at different points of $S$), the spectra of the shape operators $\mc{A}_\upxi$ and $\mc{A}_\upnu$ coincide. This is a simple consequence of the facts that $S$ is a homogeneous submanifold and that the slice representation of the action at any point of $S$ is transitive on the unit sphere in the normal space to $S$ at that point. Submanifolds with this noteworthy geometric property were investigated and called \emph{CPC submanifolds} in~\cite{berndt_SL_CPC}. In fact, one of the goals of that article was to show that singular orbits of C1-actions are far from being the only class of submanifolds that enjoy the CPC property.
